Deep Metric Learning via Facility Location

Learning the representation and the similarity metric in an end-to-end fashion with deep networks have demonstrated outstanding results for clustering and retrieval. However, these recent approaches still suffer from the performance degradation stemming from the local metric training procedure which is unaware of the global structure of the embedding space. We propose a global metric learning scheme for optimizing the deep metric embedding with the learnable clustering function and the clustering metric (NMI) in a novel structured prediction framework. Our experiments on CUB200-2011, Cars196, and Stanford online products datasets show state of the art performance both on the clustering and retrieval tasks measured in the NMI and Recall@K evaluation metrics.

==> rel.tex <==
\section{Related works}
This paper is closely related to the following active research areas: 

\noindent\textbf{Deep metric learning:}~
The seminal work in deep metric learning is the contrastive embedding with siamese network \cite{contrastive, faceVerification} where the task is to minimize the pairwise distance between a pair of examples with the same class labels and to push the pairwise distance between a pair of examples with different class labels at least greater than some fixed margin constant. On the other hand, metric learning with triplet loss \cite{triplet, triplet-svm} first constructs triplets (a triplet has \emph{anchor}, \emph{positive}, \emph{negative} where the anchor and the positive have the same class labels and the negative has the different class label) and tries to place the anchor and positive closer than the distance between the anchor and the negative with some fixed margin.

\noindent\textbf{Hard negative mining in mini-batch SGD:}~
In practice, however, the performance of these methods depends highly on the pair and the triplet sampling strategy. FaceNet \cite{facenet} suggested the \emph{semi-hard} online hard negative mining strategy where each positive pair within the mini batch actively selects which negative example to use to construct the triplet. Lifted structured embedding \cite{liftedstruct} work proposed a smooth and differentiable strategy for online hard negative sampling with convex objective. 

\noindent\textbf{Deep clustering:}~
Recently, there has been some literature \cite{deepclustering, matrixbackprop} on learning to cluster with deep networks. \cite{deepclustering} uses Frobenius norm on the residual between the binary ground truth and estimated pairwise affinity matrix for speech spectrogram signal clustering but directly estimating the binary affinity matrix with Frobenius norm is unlikely to work for pixel based images. Matrix backpropagation \cite{matrixbackprop} employ differentiable second-order pooling and normalized cuts for image segmentation. However, this approach requires computing the eigenvalue decomposition of the data matrix which has the cubic time complexity and is not very practical for moderate sized problems.\\

The paper is organized as follows. In section \ref{sec:metric_review}, we review some of the state of art methods in deep metric learning. In section \ref{sec:methods} we discuss our proposed approach. Then, we describe the implementation details \ref{sec:implementation} for reproducibility of the experiments. We show the quantitative and qualitative results in section \ref{sec:experiments} and conclude in section \ref{sec:conclusion}.


==> review.tex <==
\section{Review of state of the art deep metric learning methods}
\label{sec:metric_review}

In this section, we briefly review some of the state of the art \cite{facenet, liftedstruct, npairs} deep metric learning methods.

\subsection{Triplet learning with semi-hard negative mining}

State of the art triplet learning \cite{facenet} methods employ ``semi-hard" negative mining strategy. The idea is to construct triplets by mining ``semi-hard" negative example in the batch which are just larger than the distance between the positive pairs or (if none exists) just smaller than the positive distance. Concretely,

\begin{align}
\begin{split}
&\ell\left(X, \mathbf{y}\right) = \frac{1}{|\mathcal{P}|}\sum_{\left(i,j\right) \in \mathcal{P}} \left[ D_{i,j}^2 + \alpha - D^2_{i,k^*\left(i, j\right)} \right]_+\\
&\text{s.t.}~~~ I_{i,j} = \mathbb{I}\left[\exists k: \mathbf{y}[k] \neq \mathbf{y}[i], ~\text{s.t.}~ D^2_{i,k} > D^2_{i,j}\right] \\
&\hspace{1.8em} k^*\left(i, j\right) = I_{i,j} \left(\argmin_{k: ~\mathbf{y}[k] \neq \mathbf{y}[i]} D^2_{i,k} ~~\text{s.t.}~ D^2_{i,k} > D^2_{i,j}\right) +\\ 
&\hspace{6em} \left(1 - I_{i,j} \right) \left( \argmax_{k: ~\mathbf{y}[k] \neq \mathbf{y}[i]} D^2_{i,k} \right),
\end{split}
\end{align}

\noindent where $\mathcal{P}$ denotes the set of pairs of examples with the same class labels. The operator $[\cdot]_+$ denotes the hinge function which takes the positive component of the argument, $\mathbb{I}[\cdot]$ is the indicator function which returns $1$ if the argument is true and $0$ otherwise and $D_{i,j}$ means the euclidean distance of the two data points $X_i$ and $X_j$ in the embedding space; $|| f(X_i) - f(X_j) ||_2$. The $\alpha$ denotes the fixed margin constant.

\subsection{Lifted structured embedding}

Song \textit{et al}. proposed lifted structured embedding \cite{liftedstruct} where each positive pair compares the distances against all the negative pairs weighted by the margin constraint violation. The idea is to have a differentiable smooth loss which incorporates the online hard negative mining functionality using the \emph{log-sum-exp} formulation.

\begin{align}
\begin{split}
\ell\left(X, \mathbf{y}\right) = \frac{1}{2|\mathcal{P}|}\sum_{\left(i,j\right) \in \mathcal{P}}& \Bigg[ \log \Bigg( \sum_{\left(i,k\right) \in \mathcal{N}} \exp \left\{\alpha - D_{i,k}\right\} +\\
&\sum_{\left(j,l\right) \in \mathcal{N}} \exp \left\{ \alpha - D_{j,l} \right\} \Bigg) + D_{i,j} \Bigg]_+^2,
\end{split}
\end{align}

\noindent where $\mathcal{N}$ denotes the set of pairs of examples with different class labels.

\subsection{N-pairs embedding}
Recently, Sohn \textit{et al}. proposed N-pairs loss \cite{npairs} which enforces softmax cross-entropy loss among the pairwise similarity values in the batch.

\begin{align}
\begin{split}
\ell\left(X, \mathbf{y}\right) = \frac{-1}{|\mathcal{P}|} \sum_{(i,j) \in \mathcal{P}} \log \frac{\exp\{S_{i,j}\}}{\exp\{S_{i,j}\} + \displaystyle\sum_{k: ~\mathbf{y}[k] \neq \mathbf{y}[i]} \exp\{S_{i,k}\}},
\end{split}
\end{align}

\noindent where means the feature dot product between two data points in the embedding space; $S_{i,j} = f(X_i)^\intercal f(X_j)$.


